ProBO: Versatile Bayesian Optimization Using Any Probabilistic Programming Language

Optimizing an expensive-to-query function is a common task in science and engineering, where it is beneficial to keep the number of queries to a minimum. A popular strategy is Bayesian optimization (BO), which leverages probabilistic models for this task. Most BO today uses Gaussian processes (GPs), or a few other surrogate models. However, there is a broad set of Bayesian modeling techniques that could be used to capture complex systems and reduce the number of queries in BO. Probabilistic programming languages (PPLs) are modern tools that allow for flexible model definition, prior specification, model composition, and automatic inference. In this paper, we develop ProBO, a BO procedure that uses only standard operations common to most PPLs. This allows a user to drop in a model built with an arbitrary PPL and use it directly in BO. We describe acquisition functions for ProBO, and strategies for efficiently optimizing these functions given complex models or costly inference procedures. Using existing PPLs, we implement new models to aid in a few challenging optimization settings, and demonstrate these on model hyperparameter and architecture search tasks.

==> old/experiments.tex <==
\vspace{-2mm}
\section{Empirical Results}
\label{sec:empiricalresults}
\vspace{-1mm}
The main goal of our empirical work is to show that we can directly plug models
implemented with various PPL implementations into \probosp, and that these PPs
can improve BO performance (i.e. increase the data efficiency and reduce the
number of iterations)  when compared with standard methods and models. We also
aim to verify that our black box acquisition functions and extensions (e.g.
multi-fidelity $\hat{a}_\text{MF}$ and BPoE ensemble) perform well in practice.

%The black box acquisition functions (Algs.~\ref{alg:ei}-\ref{alg:ts}), in
%conjunction with the multi-fidelty wrapper (Alg.~\ref{alg:mf}), allow for accurate
%BO when used in place of exact aquisition functions.

We show experimental results on two tasks. The first is the task of
\emph{corrupt BO}, where we assume experimental observations $y$ are corrupted
(i.e. drawn from some corruption distribution) according to some probability.
To perform accurate BO in this setting, models need to infer when to ignore or
use subsets of the data.

The second experiment is a model selection task in neural networks that
involves finding the optimal number of hidden units at each layer in a network
(i.e a basic type of neural architecture search \cite{zoph2016neural,
kandasamy2018neural}). To reduce the number of iterations needed in BO, we
design a basin model that captures the relationship of validation error (i.e.
classification error on a validation data set) with model complexity, and
combine it with a GP in a BPoE ensemble (Sec.~\ref{sec:bpoe}).


\paragraph{Implementation Details.}
For all GP implementations in the following experiments, we use the GPy library
\cite{gpy2014}. We implement other PPs in Edward \cite{tran2016edward}, where
we use black box variational inference algorithms, and in Stan
\cite{carpenter2015stan}, where we use the No U-Turn Sampler
\cite{hoffman2011no}, a form of Hamiltonian Monte Carlo.





\vspace{-2mm}
\subsection{Corrupt BO}
\label{sec:corruptbo}
\vspace{-1mm}


% CORRUPT BO ILLUSTRATION FIGURE
\insertFigCorruptBo

Consider the setting where, each time we conduct an experiment, we observe a
``corrupt'' output $y\in\mathcal{Y}$ with probability $p$, which is drawn
according to some corruption distribution. We call this task \emph{corrupt BO}.
The corrupt distribution may have some dependence on input $\mathcal{X}$ (e.g.
$p$ may be greater in a window around the optimum value $x^*$).

% E1 EXPERIMENT FIGURE
\insertFigEOne

We develop a \emph{denoising PP} model for this setting. Given
a PP system model $p_s$, and corruption model $p_c$, we write our model as
$y \sim w_s p_s(\cdot|z_s;x) + w_c p_c(\cdot|z_c;x)$,
where 
$z_s, z_c \sim \text{Prior}(\cdot)$, and 
$w_s, w_c \sim \text{Prior}(\cdot|x)$.
%\begin{align}
  %z_s, z_c &\sim \text{Prior}(\cdot), \hspace{2mm} w_s, w_c \sim \text{Prior}(\cdot|x) \nonumber \\
  %y &\sim w_s p_s(\cdot|z_s;x) + w_c p_c(\cdot|z_c;x).
%\end{align}
%\begin{align}
  %z_s, z_c &\sim \text{Prior}(\cdot)\\
  %w_s, w_c &\sim \text{Prior}(\cdot|x)\\
  %y &\sim w_s p_s(\cdot|z_s;x) + w_c p_c(\cdot|z_c;x).
%\end{align}
This is a two component mixture of the system and a corruption model
where weights $(w_s,w_c)$ can also depend on input $x$.


% E2 NAS FIGURE
\insertFigETwo


% E3 MF FIGURE
\insertFigEThree


As a special case of this, we implement a denoising GP model, which we
illustrate in Fig.~\ref{fig:corruptbo}. Here, we let the system model $p_s$ be
a GP, and the corruption model $p_c$ be the $\text{Unif}([-10,10])$ uniform
distribution.

We show experimental results for \probosp using denoising GPs in the following
synthetic corrupt BO task. For an $x \in \mathbb{R}^d$, with probability $1-p$
we query the function $f(x)$ $=$ $ \norm{x}_2-\frac{1}{d}\sum_{i=1}^d \text{cos}(x_i)$,
%\begin{align*}
  %f(x) =  \norm{x}_2-\frac{1}{d}\sum_{i=1}^d \text{cos}(x_i),
%\end{align*}
which has a minimum value of $f(x^*)=-1$ at $x^* = 0_d$,
and with probability $p$, we receive a corrupt value with distribution
$f(x)$ $\sim$ $\text{Unif}([f_\text{max}/10,f_\text{max}])$,
%\begin{align*}
  %f(x) \sim \text{Unif}([f_\text{max}/10,f_\text{max}])
%\end{align*}
where $f_\text{max}$ is $\max_{x\in \mathcal{X}} f(x)$. Note that we use this
corruption distribution (where corruption output is  greater or equal to the
minimum $f(x^*)$) so that we are consistent with our stated goal to minimize
$y_n^0$, the observed value of the system in $\mathbb{R}$ at iteration $n$,
instead of operating in a more general design of experiments setting
\cite{kandasamy2018myopic}.

For this task we compare \probosp using denoising GPs and black box acquisition
functions with standard BO using GPs and exact acquisition functions.  We first
show results for a low corruption setting $(p=1/100)$, in
Fig.~\ref{fig:e1}(a-b), where we plot the minimal found value $y_{\min}$ $=$
$\min_{t\leq n} y_t^0$ vs iteration $n$. All methods are averaged over 10 runs,
and error bars represent one standard error. Here, both models 
converge to a near-optimal value and perform similarly.

We then show results for a high corruption setting $(p=1/3)$, in
Fig.~\ref{fig:e1}(c-d).  Here, \probosp with denoising GPs converges to a
near-optimal value, while standard BO with GPs does not. For large $n$, BO with
GPs fares worse than random sampling (RAND).

 

\vspace{-2mm}
\subsection{Tuning Neural Architectures}
\label{sec:nas}
\vspace{-1mm}
A popular application of BO is hyperparameter tuning of machine learning
models.  A recently popular task in this domain is known as neural archicture
search (NAS). In this experiment we show that domain knowledge of features of a
function landscape can be incoporated in \probosp via a BPoE ensemble
(Sec.~\ref{sec:bpoe}) to provide better sample efficiency (reduced iterations) for
BO, in a basic NAS task.

When modeling datasets of moderate size, there are often two distinct phases as
model complexity grows: a phase where the model underfits, where increasing
modeling complexity reduces error on a held-out validation set; and a phase
where the model overfits, where validation error increases with respect to
model complexity. We design a model for this trend, which we refer to as a
basin model:
\begin{align}
  y \sim \mathcal{N}(R(x-\mu;a,b)+c,\sigma^2),
\end{align}
where $R(x;a,b)$ $=$ $a^T \text{ReLU}(x) + b^T \text{ReLU}(-x)$, and we've
placed priors on parameters $\mu\in \mathbb{R}_d$, $a, b\in\mathbb{R}_d^+$,
$c\in \mathbb{R}$, and $\sigma^2>0$. This model captures the inflection point
with variable $\mu$, and uses variables $a$ and $b$ to model the slope of the
optimization landscape above and below (respectively) $\mu$.  We show a one
dimensional view of validation error data from this system, and illustrate the
basin model, in Fig.~\ref{fig:nas}(a-b).

In this experiment, we optimize over the number of units (i.e. layer width) of
the hidden layers in a four layer multi-layer perceptron (MLP) neural network
\cite{rosenblatt1961principles}, trained on the Wisconsin Breast Cancer
Diagnosis dataset \cite{blake1998uci}. We compare \probosp using a BPoE
ensemble (Sec.~\ref{sec:bpoe}) of a basin model and a GP, with
standard BO using a GP. We see in Fig~\ref{fig:nas}(c-d) that \probosp with the
BPoE ensemble can significantly outperform standard BO with GPs.  In this
optimization task, the landscape around the inflection point (of under to over
fitting) can be very steep, which may hurt the performance of standard BO with
GPs. In contrast, the basin model can capture this shape and quickly identify
the inflection point via inferences about $\mu$.


\vspace{-2mm}
\subsection{Multi-fidelity Acquisition Optimization}
\label{sec:mfexp}
\vspace{-1mm}
Here, we empirically assess our multi-fidelity acquisition function
optimization algorithm (Sec.~\ref{sec:mf}). Our goal is to demonstrate that
increasing the fidelity $M$ in black box acquisitions can yield better
performance in \probosp, and that our multi-fidelity method (Alg.~\ref{alg:mf})
maintains the performance of the high-fidelity acquisitions while reducing the
number of calls to \texttt{pp.gen}.

We perform an experiment in a two-fidelity setting, where $M \in \{10,1000\}$,
and we apply our multi-fidelity method to BB-EI and BB-UCB, using a GP model
and the synthetic BO task described in Sec.~\ref{sec:corruptbo}. Results are
shown in Fig.~\ref{fig:mf}, where we compare high-fidelity $\hat{a}$ ($M =
1000$), low-fidelity $\hat{a}$ ($M=10$), and multi-fidelity
$\hat{a}_\text{MF}$, for BB-EI (a) and BB-UCB (b).  For both black box
acquisition functions, the high-fidelity and multi-fidelity methods show
comparable performance, while the low-fidelity method performs worse. We also
see in (c) that the multi-fidelity method reduces the number of calls to
\texttt{pp.gen} by a factor of 3, on average, relative to the high fidelity
method. It is worth noting that the low-fidelity method performs well, given
its low cost, and may be the most applicable method depending on the PP noise,
cost of calling \texttt{pp.gen}, and desired accuracy.


==> old/experiments_figonly.tex <==
% CORRUPT BO ILLUSTRATION FIGURE
\insertFigCorruptBo

% E1 EXPERIMENT FIGURE
\insertFigEOne

% E2 NAS FIGURE
\insertFigETwo

% E3 MF FIGURE
\insertFigEThree


==> old/figure_mfacqopt_old.tex <==
%\newlength{\minipagewidth}
%\newlength{\minipageoffset}
%\newlength{\columngap}
%\newlength{\pretitlegap}
%\newlength{\posttitlegap}

\setlength{\minipagewidth}{0.43\textwidth}
\setlength{\minipageoffset}{0mm}
\setlength{\columngap}{2mm}
\setlength{\pretitlegap}{2mm}
\setlength{\posttitlegap}{3mm}

\begin{figure}[bp]
  \centering

  \begin{minipage}[b]{\textwidth}
    \centering
    \vspace{\pretitlegap}
    \textbf{Multifidelity Acquisition Functions}
    \vspace{\posttitlegap}
  \end{minipage}\\

  \begin{minipage}[b]{\minipagewidth}
    \hspace{\minipageoffset}
    \centering
    {\small (a) EI}
  \end{minipage}
  \hspace{\columngap}
  \begin{minipage}[b]{\minipagewidth}
    \hspace{\minipageoffset}
    \centering
    {\small (b) UCB}
  \end{minipage}\\

  \begin{minipage}[b]{\minipagewidth}
    \includegraphics[width=\textwidth]{fig/e3_f1}
  \end{minipage}
  \hspace{\columngap}
  \begin{minipage}[b]{\minipagewidth}
    \includegraphics[width=\textwidth]{fig/e3_f2}
  \end{minipage}\\

  \begin{minipage}[b]{.9\minipagewidth}
    \hspace{\minipageoffset}
    \centering
    {\small (c) Calls to \texttt{gen}}
  \end{minipage}\\

  \begin{minipage}[b]{.9\minipagewidth}
    \centering
    \includegraphics[width=\textwidth]{fig/mftable4}
  \end{minipage}\\

  \caption{
    Results on $a_\text{MF}$ experiments (Sec.~\ref{sec:mfexp}), showing
    (a)-(b) \probosp using $a_\text{MF}$ (Alg.~\ref{alg:mf}) vs using a fixed
    high-fidelity $a$ ($M=1000$) and a fixed low-fidelity $a$ ($M=10$). Here,
    $a_\text{MF}$ performs competitively with the high-fidelity $a$, while low
    fidelity $a$ performs worse. In (c) we show the average number of
    \texttt{post}/\texttt{gen} calls per evaluation of $a$.  We see that the
    $a_\text{MF}$ reduces the number of calls.
    Curves are averaged over 10 trials, and error bars represent one standard
    error.
    \label{fig:mfacqopt}
  }
\end{figure}


==> old/figure_multitask_old.tex <==
%\newlength{\minipagewidth}
%\newlength{\minipageoffset}
%\newlength{\columngap}
%\newlength{\pretitlegap}
%\newlength{\posttitlegap}

\setlength{\minipagewidth}{0.43\textwidth}
\setlength{\minipageoffset}{0mm}
\setlength{\columngap}{2mm}
\setlength{\pretitlegap}{2mm}
\setlength{\posttitlegap}{3mm}

\begin{figure}[bp]
  \centering

  \begin{minipage}[b]{\textwidth}
    \centering
    \vspace{\pretitlegap}
    \textbf{Structured Multi-task BO}
    \vspace{\posttitlegap}
  \end{minipage}\\

  \begin{minipage}[b]{\minipagewidth}
    \hspace{\minipageoffset}
    \centering
    {\small (a) GP (two task)}
  \end{minipage}
  \hspace{\columngap}
  \begin{minipage}[b]{\minipagewidth}
    \hspace{\minipageoffset}
    \centering
    {\small (b) Warp model (two task)}
  \end{minipage}\\

  \begin{minipage}[b]{\minipagewidth}
    \includegraphics[width=\textwidth]{fig/e5_viz01}
  \end{minipage}
  \hspace{\columngap}
  \begin{minipage}[b]{\minipagewidth}
    \includegraphics[width=\textwidth]{fig/e5_viz02}
  \end{minipage}\\

  \begin{minipage}[b]{\minipagewidth}
    \hspace{\minipageoffset}
    \centering
    {\small (c) EI}
  \end{minipage}\\

  \begin{minipage}[b]{\minipagewidth}
    \includegraphics[width=\textwidth]{fig/e5_f1}
  \end{minipage}\\

  \caption{
    Structured multi-task BO (Sec.~\ref{sec:multitask_and_ensembles}). We show
    (a) independent GPs and (b) our warp model, in a two-task setting.
    In (c) we show results for structured multi-task BO (details in Appendix
    Sec.~\ref{sec:multitaskbo}).  Curves are averaged over 10 trials, and error
    bars represent one standard error.
    \label{fig:multitask}
  }
\end{figure}


==> old/figure_pplacq_old.tex <==
% SETTING COLUMNNAME, COLUMNNAMELEFT, TEMPHEIGHT, TEMPWIDTH, PLOTWIDTHTHIRD, PLOTWIDTHQUARTER, BETWEENSPACE, LEFTSPACE
\newlength{\tempheight}
\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\tempheight][c]{#1}}}

\newlength{\tempwidth}
\newcommand{\columnname}[1]% #1 = text
{\makebox[\tempwidth][c]{#1}}
\newcommand{\columnnameleft}[1]% #1 = text
{\makebox[\tempwidth][l]{#1}}


\newcommand{\plotwidthThird}{0.3\textwidth} 
%\newcommand{\plotwidthQuarter}{0.25\textwidth} 
\newcommand{\plotwidthQuarter}{0.25\textwidth} 
\newcommand{\plotwidthOneColHalf}{0.23\textwidth} 
\newcommand{\betweenspace}{\hspace{-0.1in}}
%\newcommand{\leftspace}{\hspace{0.0in}}
\newcommand{\leftspace}{\hspace{-5mm}}











% PPL ACQUISITIONS FIGURE
\begin{figure*}

\setlength{\tempwidth}{0.25\textwidth}
\settoheight{\tempheight}{\includegraphics[width=\tempwidth]{fig/bbacq00}}%
\begin{center}
%\columnnameleft{(a)\hspace{3mm}$a_\text{EI}(x)$ (Alg.~\ref{alg:ei})}
%\betweenspace
%\columnnameleft{(b)\hspace{3mm}$a_\text{PI}(x)$ (Alg.~\ref{alg:pi})}
%\betweenspace
%\columnnameleft{\hspace{1mm}(c)\hspace{3mm}$a_\text{UCB}(x)$ (Alg.~\ref{alg:ucb})}
%\betweenspace
%\columnnameleft{\hspace{2mm}(d)\hspace{3mm}$a_\text{TS}(x)$ (Alg.~\ref{alg:ts})}
%
%\columnnameleft{(a)\hspace{1mm}$a_\text{EI}(x, \texttt{post}, \texttt{gen})$}
%\betweenspace
%\columnnameleft{(b)\hspace{1mm}$a_\text{PI}(x, \texttt{post}, \texttt{gen})$}
%\betweenspace
%\columnnameleft{\hspace{1mm}(c)\hspace{1mm}$a_\text{UCB}(x, \texttt{post}, \texttt{gen})$}
%\betweenspace
%\columnnameleft{\hspace{2mm}(d)\hspace{1mm}$a_\text{TS}(x, \texttt{post}, \texttt{gen})$}
%
\leftspace
\hspace{1mm}
\columnnameleft{(a)\hspace{8mm}$a_\text{EI}(x)$}
\betweenspace
\hspace{1mm}
\columnnameleft{(b)\hspace{8mm}$a_\text{PI}(x)$}
\betweenspace
\hspace{1mm}
\columnnameleft{(c)\hspace{8mm}$a_\text{UCB}(x)$}
\betweenspace
\hspace{1mm}
\columnnameleft{(d)\hspace{8mm}$a_\text{TS}(x)$}
\vspace{-0.1in}

\leftspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/bbacq01}
\label{fig:bbacq1}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/bbacq00}
\label{fig:bbacq2}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/bbacq02}
\label{fig:bbacq3}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/bbacq03}
\label{fig:bbacq4}}

\vspace{-0.05in}
\caption{
\small 
Visualizations of PPL acquisition functions $a(x)$ given in
Algs.~\ref{alg:ei}-\ref{alg:ts} for use in \probo. In each plot, the data and
posterior predictive distribution are shown, and $a(x)$ is given for two
fidelities: $M=50$ (solid color line) and $M=500$ (dashed black line).
\label{fig:bbacq}
}
\end{center}
\end{figure*}


==> old/figures.tex <==
% SETTING COLUMNNAME, COLUMNNAMELEFT, TEMPHEIGHT, TEMPWIDTH, PLOTWIDTHTHIRD, PLOTWIDTHQUARTER, BETWEENSPACE, LEFTSPACE
\newlength{\tempheight}
\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\tempheight][c]{#1}}}

\newlength{\tempwidth}
\newcommand{\columnname}[1]% #1 = text
{\makebox[\tempwidth][c]{#1}}
\newcommand{\columnnameleft}[1]% #1 = text
{\makebox[\tempwidth][l]{#1}}


\newcommand{\plotwidthThird}{0.3\textwidth} 
%\newcommand{\plotwidthQuarter}{0.25\textwidth} 
\newcommand{\plotwidthQuarter}{0.25\textwidth} 
\newcommand{\plotwidthOneColHalf}{0.23\textwidth} 
\newcommand{\betweenspace}{\hspace{-0.1in}}
%\newcommand{\leftspace}{\hspace{0.0in}}
\newcommand{\leftspace}{\hspace{-5mm}}











% PPL ACQUISITIONS FIGURE
\newcommand{\insertFigAcq}{ 

\begin{figure*}

\setlength{\tempwidth}{0.25\textwidth}
\settoheight{\tempheight}{\includegraphics[width=\tempwidth]{fig/bbacq00}}%
\begin{center}
%\columnnameleft{(a)\hspace{3mm}$a_\text{EI}(x)$ (Alg.~\ref{alg:ei})}
%\betweenspace
%\columnnameleft{(b)\hspace{3mm}$a_\text{PI}(x)$ (Alg.~\ref{alg:pi})}
%\betweenspace
%\columnnameleft{\hspace{1mm}(c)\hspace{3mm}$a_\text{UCB}(x)$ (Alg.~\ref{alg:ucb})}
%\betweenspace
%\columnnameleft{\hspace{2mm}(d)\hspace{3mm}$a_\text{TS}(x)$ (Alg.~\ref{alg:ts})}
%
%\columnnameleft{(a)\hspace{1mm}$a_\text{EI}(x, \texttt{post}, \texttt{gen})$}
%\betweenspace
%\columnnameleft{(b)\hspace{1mm}$a_\text{PI}(x, \texttt{post}, \texttt{gen})$}
%\betweenspace
%\columnnameleft{\hspace{1mm}(c)\hspace{1mm}$a_\text{UCB}(x, \texttt{post}, \texttt{gen})$}
%\betweenspace
%\columnnameleft{\hspace{2mm}(d)\hspace{1mm}$a_\text{TS}(x, \texttt{post}, \texttt{gen})$}
%
\leftspace
\hspace{1mm}
\columnnameleft{(a)\hspace{8mm}$a_\text{EI}(x)$}
\betweenspace
\hspace{1mm}
\columnnameleft{(b)\hspace{8mm}$a_\text{PI}(x)$}
\betweenspace
\hspace{1mm}
\columnnameleft{(c)\hspace{8mm}$a_\text{UCB}(x)$}
\betweenspace
\hspace{1mm}
\columnnameleft{(d)\hspace{8mm}$a_\text{TS}(x)$}
\vspace{-0.1in}

\leftspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/bbacq01}
\label{fig:bbacq1}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/bbacq00}
\label{fig:bbacq2}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/bbacq02}
\label{fig:bbacq3}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/bbacq03}
\label{fig:bbacq4}}

\vspace{-0.05in}
\caption{
\small 
Visualizations of PPL acquisition functions $a(x)$ given in
Algs.~\ref{alg:ei}-\ref{alg:ts} for use in \probo. In each plot, the data and
posterior predictive distribution are shown, and $a(x)$ is given for two
fidelities: $M=50$ (solid color line) and $M=500$ (dashed black line).
\label{fig:bbacq}
}
\end{center}
\end{figure*}
}









% ALL VIZ / ALL ILLUSTRATIONS COMBINED
\newcommand{\insertFigAllViz}{ 

\begin{figure*}

\setlength{\tempwidth}{0.26\textwidth}

\settoheight{\tempheight}{\includegraphics[width=\tempwidth]{fig/corruptbo_01}}%
\begin{center}

% STATES/NANVALS (e4)
\begin{flushleft}
\hspace{-2mm} \underline{\textbf{BO with State Observations}}\\
\end{flushleft}
%\vspace{-0.05in}
\leftspace
\columnnameleft{\hspace{2mm} \small (a) Data and true mean}
\betweenspace
\columnnameleft{\hspace{3mm} \small (b) GP (state 1 data)}
\betweenspace
\columnnameleft{\hspace{2mm} \small (c) GP (all data)}
\betweenspace
\columnnameleft{\hspace{2mm} \small (d) Switching (all data)}
\\
\vspace{-0.15in}

\leftspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e4_viz01}
\label{fig:e4viz01}}
\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e4_viz02}
\label{fig:e4viz02}}
\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e4_viz03}
\label{fig:e4viz03}}
\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e4_viz04}
\label{fig:e4viz04}}
\\


% CONTAMINATED
\vspace{-3mm}
\begin{flushleft}
\hspace{-2mm} \underline{\textbf{Contaminated BO}}\\
\end{flushleft}
\vspace{-0.05in}
\leftspace
\columnnameleft{\hspace{1mm} \small (a)  GP ($n=20$)}
\betweenspace
\columnnameleft{\hspace{2mm} \small (b)  GP ($n=50$)}
\betweenspace
\columnnameleft{\hspace{1mm} \small (c) Denoising ($n=20$)}
\betweenspace
\columnnameleft{\hspace{1mm} \small (d) Denoising ($n=50$)}
\\
\vspace{-0.15in}

\leftspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/corruptbo_01}
\label{fig:corruptbo1}}
\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/corruptbo_03}
\label{fig:corruptbo3}}
\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/corruptbo_02}
\label{fig:corruptbo2}}
\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/corruptbo_04}
\label{fig:corruptbo4}}
\\


% BASIN (prior structure) and Multi-task / Warping (e5)
\vspace{-2mm}
\begin{flushleft}
\hspace{-2mm} \underline{\smash{\textbf{BO with Prior Structure on Objective}}}\hspace{8mm}
\underline{\textbf{Structured Multi-task BO}} \\
\end{flushleft}
\vspace{-0.05in}
\leftspace
\columnnameleft{\hspace{2mm} \small (a) GP}
\betweenspace
\columnnameleft{\hspace{3mm} \small (b) Basin}
\betweenspace
\columnnameleft{\hspace{2mm} \small (c) GP (two task)}
\betweenspace
\columnnameleft{\hspace{1mm} \small (d) Warp (two task)}
\\
\vspace{-0.15in}

\leftspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/basin_nas_01}
\label{fig:basinnas01}}
\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/basin_nas_02}
\label{fig:basinnas02}}
\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e5_viz01}
\label{fig:e5viz01}}
\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e5_viz02}
\label{fig:e5viz02}}

\vspace{-0.05in}
\caption{
\small 
Inference results on models developed in Sec.~\ref{sec:examples}.
\textbf{Row 1:} BO with state observations. We show (a) the true function, (b)
a GP model fit on state 1 data only, (c) the same GP model fit on all data, where
hyperparameter estimates are badly influenced, and (d) our switching model.
\textbf{Row 2:} Contaminated BO. We show (a) inference in a GP with n=20
and (b) n=50, and (c-d) inference in our denoising version of the same GP.
\textbf{Row 3 (a-b):} Basin model for overfitting. We plot validation accuracy
vs layer width for a small dataset, and show inference in (a) a GP and (b) our
basin model.
%\textbf{Row 3 (a-b):} Structure on objective. For a small set of model complexity
%data, we show (a) a GP and (b) our basin model.
\textbf{Row 3 (c-d):} Structured multi-task BO. We show (a) independent GPs and
(b) our warp model, in a two-task setting.
\label{fig:allviz}
}
\end{center}
\end{figure*}
}













% ALL RESULTS / All CURVES PLOTS COMBINED
\newcommand{\insertFigAllCurves}{ 

\begin{figure*}

\setlength{\tempwidth}{0.26\textwidth}

\settoheight{\tempheight}{\includegraphics[width=\tempwidth]{fig/corruptbo_01}}%
\begin{center}


% NAS/Model Complexity Results Plots
\begin{flushleft}
\hspace{-2mm} \underline{\textbf{BO with State Observations}}
\hspace{20mm} \underline{\smash{\textbf{BO with Prior Structure on Objective}}}\\
\end{flushleft}
%\vspace{-0.05in}
\leftspace
\columnnameleft{\hspace{2mm} \small (a) EI and UCB}
\betweenspace
\columnnameleft{\hspace{3mm} \small (b) PI and TS}
\betweenspace
\columnnameleft{\hspace{2mm} \small (c) EI and UCB}
\betweenspace
\columnnameleft{\hspace{1mm} \small (d) PI and TS}
\\
\vspace{-0.15in}
%
%\leftspace
%\columnnameleft{\hspace{2mm}(a)  title}
%\betweenspace
%\columnnameleft{\hspace{3mm}(b)  title}
%\betweenspace
%\columnnameleft{\hspace{4mm}(c)  title}
%\betweenspace
%\columnnameleft{\hspace{5mm}(d)  title}
%\\
%\vspace{-0.15in}

\leftspace
\subfloat{
\includegraphics[width=\plotwidthQuarter-1mm]{fig/e4_f1}
\label{fig:e4f1}}
\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter-1mm]{fig/e4_f2}
\label{fig:e4f2}}
\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e2_f1_01}
\label{fig:nas1}}
\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e2_f2_01}
\label{fig:nas2}}
\\
\vspace{-0.1in}


% Contaminated BO Results Plots
\begin{flushleft}
\hspace{-2mm} \underline{\textbf{Contaminated BO}}\\
\end{flushleft}
\vspace{-0.05in}
\leftspace
\columnnameleft{\hspace{2mm} \small (a) EI and UCB ($p=.01$)}
\betweenspace
\columnnameleft{\hspace{3mm} \small (b) PI and TS ($p=.01$)}
\betweenspace
\columnnameleft{\hspace{2mm} \small (c) EI and UCB ($p=.33$)}
\betweenspace
\columnnameleft{\hspace{3mm} \small (d) PI and TS ($p=.33$)}
\\
\vspace{-0.15in}
%
%\leftspace
%\columnnameleft{\hspace{2mm}(a)  title}
%\betweenspace
%\columnnameleft{\hspace{3mm}(b)  title}
%\betweenspace
%\columnnameleft{\hspace{4mm}(c)  title}
%\betweenspace
%\columnnameleft{\hspace{5mm}(d)  title}
%\\
%\vspace{-0.15in}

\leftspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e1_f1_2}
\label{fig:combine1}}
\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e1_f2_2}
\label{fig:combine2}}
\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e1_f1_1}
\label{fig:combine3}}
\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e1_f2_1}
\label{fig:combine3}}
\\
\vspace{-0.1in}


% MF (multi-fidelity) acquisition plots 
%\begin{flushleft}
%\hspace{18mm} \underline{\textbf{Multifidelity Acquisition Functions}}\\
%\end{flushleft}
%\vspace{-0.05in}
%%\leftspace
%\columnnameleft{\hspace{2mm}(a)  title}
%\betweenspace
%\columnnameleft{\hspace{3mm}(b)  title}
%\betweenspace
%\columnnameleft{\hspace{4mm}(c)  title}
%%\betweenspace
%%\columnnameleft{\hspace{5mm}(d)  title}
%\\
%\vspace{-0.15in}

%%\leftspace
%\subfloat{\includegraphics[width=\plotwidthQuarter]{fig/e3_f1}
%\label{fig:mf1}}
%%\betweenspace
%\subfloat{\includegraphics[width=\plotwidthQuarter]{fig/e3_f2}
%\label{fig:mf2}}
%%\betweenspace
%\subfloat{
%%\includegraphics[height=\tempheight-0.24in]{fig/mftable2}
%\includegraphics[width=\plotwidthQuarter]{fig/mftable3}
%\label{fig:mf3}}

\begin{flushleft}
\hspace{-2mm} \underline{\textbf{Multifidelity Acquisition Functions}}
\hspace{10mm} \underline{\smash{\textbf{Structured Two-Task BO}}}\\
\end{flushleft}
\vspace{-0.05in}
\leftspace
\columnnameleft{\hspace{2mm} \small (a) EI}
\betweenspace
\columnnameleft{\hspace{3mm} \small (b) UCB}
\betweenspace
\columnnameleft{\hspace{1mm} \small (c) Calls to \texttt{gen}}
\betweenspace
\columnnameleft{\hspace{5mm} \small (d) EI}
\\
\vspace{-0.15in}

\leftspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e3_f1}
\label{fig:mf1}}
\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e3_f2}
\label{fig:mf2}}
%\betweenspace
\hspace{-.07in}
\subfloat{
\includegraphics[height=\tempheight-0.12in]{fig/mftable4}
%\includegraphics[width=\plotwidthQuarter-2.5mm]{fig/mftable4}
\label{fig:mf3}}
%\betweenspace
\hspace{-.09in}
\subfloat{
\includegraphics[width=\plotwidthQuarter-2mm]{fig/e5_f1}
\label{fig:multitask1}}

\vspace{-0.05in}
\caption{
\small 
\textbf{Row 1:}
In (a-c) we show results of neural network architecture and hyperparameter
search with timeouts (Sec.~\ref{sec:exstate}), comparing \probosp using a 
switching model with BO using GPs.
In (c-d) we show results of model complexity hyperparameter tuning experiments
(Sec.~\ref{sec:nas}), comparing \probosp using a basin model with BO
using GPs.
%\label{fig:nas}
\textbf{Row 2:} Results on contaminated BO (Sec.~\ref{sec:excontam}). (a-b) For low
corruption ($p=.01$), \probosp using denoising GPs is competitive with
standard BO using GP models. (c-d) For higher corruption ($p=.33$), \probosp
converges to the optimal value, while standard BO does not, even as $n$ grows.
%Under high contamination level, standard BO can fare worse than
%RAND (blue dotted line) (c-d).
%\label{fig:e1}
\textbf{Row 3:}
Results on $a_\text{MF}$ experiments (Sec.~\ref{sec:mfexp}), showing (a-b)
\probosp using $a_\text{MF}$ (Alg.~\ref{alg:mf}) vs using a fixed high-fidelity
$a$ ($M=1000$) and a fixed low-fidelity $a$ ($M=10$). Here, $a_\text{MF}$
performs competitively with the high-fidelity $a$, while low fidelity $a$
performs worse. In (c) we show the average number of \texttt{post}/\texttt{gen}
calls per evaluation of $a$.  We see that the $a_\text{MF}$ reduces the number
of calls. In (d) we show results for structured two-task BO (Appendix
Sec.~\ref{sec:multitaskbo}).
\label{fig:mf}
\textbf{Overall:}
All curves are averaged over 10 trials, and error bars represent one standard
error.
\label{fig:allcurves}
}
\end{center}
\end{figure*}
}






















% STATES/SWTCHING MODEL (NANs, NANVALs, FAILURES) VIZ
\newcommand{\insertFigStatesViz}{ 

\begin{figure*}

\setlength{\tempwidth}{0.25\textwidth}

\settoheight{\tempheight}{\includegraphics[width=\tempwidth]{fig/corruptbo_01}}%
\begin{center}
\columnnameleft{\hspace{2mm}(a)  title}
\betweenspace
\columnnameleft{\hspace{4mm}(b)  title}
\betweenspace
\columnnameleft{\hspace{2mm}(c)  title}
\betweenspace
\columnnameleft{\hspace{5mm}(d)  title}\\
\vspace{-0.15in}

\leftspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e4_viz01}
\label{fig:corruptbo1}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e4_viz02}
\label{fig:corruptbo2}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e4_viz03}
\label{fig:corruptbo3}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e4_viz04}
\label{fig:corruptbo4}}\betweenspace
\vspace{-0.1in}
\caption{
\small 
Caption.
\label{fig:statesviz}
}
\end{center}
\end{figure*}
}












% CONTAMINATED/CORRUPT BO VIZ/ILLUSTRATION FIGURE
\newcommand{\insertFigContaminatedBo}{ 

\begin{figure*}

%\setlength{\tempwidth}{0.5\textwidth}
\setlength{\tempwidth}{0.25\textwidth}

\settoheight{\tempheight}{\includegraphics[width=\tempwidth]{fig/corruptbo_01}}%
\begin{center}
%\columnnameleft{(a)\hspace{0.25\tempwidth}\hspace{-1mm}GP ($n=20$)}
%\betweenspace
%\columnnameleft{\hspace{1mm}(b)\hspace{1mm} Denoising GP ($n=20$)}
%\betweenspace
%\columnnameleft{\hspace{2mm}(c)\hspace{0.25\tempwidth}\hspace{-1mm}GP ($n=50$)}
%\betweenspace
%\columnnameleft{\hspace{2mm}(d)\hspace{1mm} Denoising GP ($n=50$)}\\
%
%\columnnameleft{\hspace{11mm}(a)  GP ($n=20$)}
%\betweenspace
%\columnnameleft{\hspace{4mm}(b)  Denoising GP ($n=20$)}
%\betweenspace
%\columnnameleft{\hspace{2mm}\hspace{0.25\tempwidth}(c)  GP ($n=50$)}
%\betweenspace
%\columnnameleft{\hspace{5mm}(d)  Denoising GP ($n=50$)}\\
%\vspace{-0.15in}
%
\columnnameleft{\hspace{2mm}(a)  title}
\betweenspace
\columnnameleft{\hspace{3mm}(b)  title}
\betweenspace
\columnnameleft{\hspace{4mm}(c)  title}
\betweenspace
\columnnameleft{\hspace{5mm}(d)  title}\\
\vspace{-0.15in}

\leftspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/corruptbo_01}
\label{fig:corruptbo1}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/corruptbo_03}
\label{fig:corruptbo3}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/corruptbo_02}
\label{fig:corruptbo2}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/corruptbo_04}
\label{fig:corruptbo4}}\betweenspace
\vspace{-0.1in}
\caption{
\small 
Visualization of the denoising model (Sec.~\ref{sec:corruptbo}) applied to GPs,
for use in corrupt BO.  When $n=20$, the GP (a) is negatively affected by
corrupt data (orange points), while the denoising GP (b) more accurately
reflects the system data (blue points).  When $n=50$, the GP (c) remains biased
by the corrupt data, while the denoising GP (d) converges to the true system
(red dashed line).  In all figures, the corruption probability is
$p=\frac{1}{3}$, and the model posterior predictive is shown in gray.
\label{fig:corruptbo}
}
\end{center}
\end{figure*}
}











% CORRUPT BO ILLUSTRATION FIGURE OLD
\newcommand{\insertFigCorruptBoOld}{ 

\begin{figure*}

%\setlength{\tempwidth}{0.5\textwidth}
\setlength{\tempwidth}{0.25\textwidth}

\settoheight{\tempheight}{\includegraphics[width=\tempwidth]{fig/corruptbo_01}}%
\begin{center}
%\columnnameleft{(a)\hspace{0.25\tempwidth}\hspace{-1mm}GP ($n=20$)}
%\betweenspace
%\columnnameleft{\hspace{1mm}(b)\hspace{1mm} Denoising GP ($n=20$)}
%\betweenspace
%\columnnameleft{\hspace{2mm}(c)\hspace{0.25\tempwidth}\hspace{-1mm}GP ($n=50$)}
%\betweenspace
%\columnnameleft{\hspace{2mm}(d)\hspace{1mm} Denoising GP ($n=50$)}\\
\columnnameleft{\hspace{11mm}(a)  GP ($n=20$)}
\betweenspace
\columnnameleft{\hspace{4mm}(b)  Denoising GP ($n=20$)}
\betweenspace
\columnnameleft{\hspace{2mm}\hspace{0.25\tempwidth}(c)  GP ($n=50$)}
\betweenspace
\columnnameleft{\hspace{5mm}(d)  Denoising GP ($n=50$)}\\
\vspace{-0.15in}

\leftspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/corruptbo_01}
\label{fig:corruptbo1}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/corruptbo_02}
\label{fig:corruptbo2}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/corruptbo_03}
\label{fig:corruptbo3}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/corruptbo_04}
\label{fig:corruptbo4}}\betweenspace
\vspace{-0.1in}
\caption{
\small 
Visualization of the denoising model (Sec.~\ref{sec:corruptbo}) applied to GPs,
for use in corrupt BO.  When $n=20$, the GP (a) is negatively affected by
corrupt data (orange points), while the denoising GP (b) more accurately
reflects the system data (blue points).  When $n=50$, the GP (c) remains biased
by the corrupt data, while the denoising GP (d) converges to the true system
(red dashed line).  In all figures, the corruption probability is
$p=\frac{1}{3}$, and the model posterior predictive is shown in gray.
\label{fig:corruptbo}
}
\end{center}
\end{figure*}
}



























% COMBINED MODELS FIGURE (ENSEMBLE)
\newcommand{\insertFigCombine}{ 

\begin{figure*}
\setlength{\tempwidth}{0.3\textwidth}
\settoheight{\tempheight}{\includegraphics[width=\tempwidth]{fig/combine01}}%

\begin{center}
\hspace{0.3in}
\columnname{Phase Shift (PS) Model}
%\hspace{-0.1in}
\betweenspace
\hspace{0.1in}
\columnname{Gaussian Process (GP)}
\betweenspace
\columnname{BPoE Ensemble (PS, GP)}\\

\vspace{-0.1in}

\leftspace
\rowname{\hspace{2mm}\underline{\parbox[c][0.2in]{0in}{}\hspace{4mm}$n$ = 2\hspace{4mm}}} \hspace{-0.1in}
\subfloat{
\includegraphics[width=\plotwidthThird]{fig/combine01}
\label{fig:combine1}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthThird]{fig/combine02}
\label{fig:combine2}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthThird]{fig/combine03}
\label{fig:combine3}}\betweenspace
\\
\vspace{-0.25in}
\leftspace
\rowname{\hspace{2mm}\underline{\parbox[c][0.2in]{0in}{}\hspace{4mm}$n$ = 50\hspace{4mm}}} \hspace{-0.1in}
\subfloat{
\includegraphics[width=\plotwidthThird]{fig/combine04}
\label{fig:combine4}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthThird]{fig/combine05}
\label{fig:combine5}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthThird]{fig/combine06}
\label{fig:combine6}}\betweenspace
\caption{
\small 
Visualization of the Bayesian product of experts (BPoE) ensemble model (column
3) of a phase shift (PS) model (column 1), defined in
Sec.~\ref{sec:phaseshift}, and a GP (column two). In the first row ($n=2$),
when $n$ is small, the BPoE ensemble more closely resembles the PS model.  In
the second row ($n=50$), when $n$ is larger, the BPoE ensemble more closely
resembles the GP model, and both accurately reflect the true landscape (red
dashed line). In all figures, the posterior predictive is shown in gray.
\label{fig:combine}
}
\end{center}
\end{figure*}
}












% E1 FIGURE (e1 corrupt bo)
\newcommand{\insertFigEOne}{ 

\begin{figure*}

\setlength{\tempwidth}{0.25\textwidth}
\settoheight{\tempheight}{\includegraphics[width=\tempwidth]{fig/e1_f1_2}}%
\begin{center}

%\columnname{(a) EI and UCB $(p=0.01)$}
%\betweenspace
%%\columnname{\hspace{1mm}(b) PI and TS $\left(p=\frac{1}{100}\right)$}
%\columnname{\hspace{1mm}(b) PI and TS $(p=0.01)$}
%\betweenspace
%\columnname{\hspace{2mm}(c) EI and UCB $(p=0.33)$}
%\betweenspace
%\columnname{\hspace{3mm}(d) PI and TS $(p=0.33)$}

%\columnname{(a) EI and UCB $\left(p=\frac{1}{100}\right)$}
\columnname{\hspace{5mm}(a) EI and UCB $\left(p=1/100\right)$}
\betweenspace
%\columnname{\hspace{1mm}(b) PI and TS $\left(p=\frac{1}{100}\right)$}
\columnname{\hspace{7mm}(b) PI and TS $\left(p=1/100\right)$}
\betweenspace
%\columnname{\hspace{2mm}(c) EI and UCB $\left(p=\frac{1}{3}\right)$}
\columnname{\hspace{9mm}(c) EI and UCB $\left(p=1/3\right)$}
\betweenspace
%\columnname{\hspace{3mm}(d) PI and TS $\left(p=\frac{1}{3}\right)$}
\columnname{\hspace{11mm}(d) PI and TS $\left(p=1/3\right)$}
\vspace{-0.15in}

\leftspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e1_f1_2}
\label{fig:combine1}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e1_f2_2}
\label{fig:combine2}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e1_f1_1}
\label{fig:combine3}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e1_f2_1}
\label{fig:combine3}}\betweenspace
\vspace{-0.1in}
\caption{
\small 
Results on corrupt BO experiments (Sec.~\ref{sec:corruptbo}). For low
corruption ($p=1/100$), \probosp with black box acquisition functions on
denoising GPs is competitive with standard BO using exact aquisition functions
on GP models (a-b). For higher corruption ($p=1/3$), \probosp with denoising
GPs converges to the optimal value, while standard BO with GPs does not, even
as $n$ grows large (c-d). Under high corruptions, standard BO with GPs can fare
worse than RAND (blue dotted line) (c-d).  All methods are averaged over 10
runs, and error bars represent one standard error.
\label{fig:e1}
}
\end{center}
\end{figure*}
}




% E2 NAS FIGURE

\newcommand{\insertFigETwo}{ 
\begin{figure*}
%\begin{figure}

\setlength{\tempwidth}{0.25\textwidth}
\settoheight{\tempheight}{\includegraphics[width=\tempwidth]{fig/e2_f1_01}}%
\begin{center}

\columnnameleft{\hspace{6mm}(a)  Basin model $(n=4)$}
\betweenspace
\columnnameleft{\hspace{13mm}(b)  GP $(n=4)$}
\betweenspace
\columnnameleft{\hspace{14mm}(c)  EI and UCB}
\betweenspace
\columnnameleft{\hspace{15mm}(d)  PI and TS}\\
\vspace{-0.15in}

\leftspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/basin_nas_02}
%\includegraphics[width=\plotwidthOneColHalf]{fig/e2_f2_01}
\label{fig:nas3}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/basin_nas_01}
%\includegraphics[width=\plotwidthOneColHalf]{fig/e2_f2_01}
\label{fig:nas4}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e2_f1_01}
%\includegraphics[width=\plotwidthOneColHalf]{fig/e2_f1_01}
\label{fig:nas1}}\betweenspace
\subfloat{
\includegraphics[width=\plotwidthQuarter]{fig/e2_f2_01}
%\includegraphics[width=\plotwidthOneColHalf]{fig/e2_f2_01}
\label{fig:nas2}}\betweenspace
\vspace{-0.1in}
\caption{
\small 
Results on neural architecture tuning experiments (Sec.~\ref{sec:nas}).  We
visualize the basin model (a) vs GP (b) on data from a four layer MLP (fixing
all layers to same width to plot $x$ in 1D).  For low $n$, the basin model
more accurately captures the shape of the function (red dashed line). In (c)
and (d) we show results of \probosp using a BPoE basin ensemble vs standard BO
with GPs.  Here, the \probosp methods outperform standard BO.  All methods are
averaged over 10 runs, and error bars represent one standard error.
\label{fig:nas}
}
\end{center}
\end{figure*}
%\end{figure}
}







% E3 MF FIGURE
\newcommand{\insertFigEThree}{ 

\begin{figure*}

\setlength{\tempwidth}{0.25\textwidth}
\settoheight{\tempheight}{\includegraphics[width=\tempwidth]{fig/e3_f1}}%
\begin{center}

\columnnameleft{\hspace{12mm}(a)  BB-EI}
\betweenspace
\columnnameleft{\hspace{13mm}(b)  BB-UCB}
\betweenspace
\columnnameleft{\hspace{9mm}(c) Calls to \texttt{pp.gen}}
\vspace{-0.15in}

\subfloat{\includegraphics[width=\plotwidthQuarter]{fig/e3_f1}
\label{fig:mf1}}
\subfloat{\includegraphics[width=\plotwidthQuarter]{fig/e3_f2}
\label{fig:mf2}}
\subfloat{
\includegraphics[height=\tempheight-0.05in]{fig/mftable}
\label{fig:mf3}}


\vspace{-0.1in}


\caption{
\small 
Results on the multi-fidelity black box acqusition function experiments
(Sec.~\ref{sec:mfexp}), showing \probosp using the multi-fidelity
$\hat{a}_\text{MF}$ (Alg.~\ref{alg:mf}) vs using a fixed high-fidelity
$\hat{a}$ ($M=1000$) and a fixed low-fidelity $\hat{a}$ ($M=10$). Results for
$\hat{a}_\text{EI}$ (BB-EI) are in (a), and $\hat{a}_\text{UCB}$ (BB-UCB) in
(b). Here, $\hat{a}_\text{MF}$ performs competitively with the high-fidelity
$\hat{a}$, while low fidelity $\hat{a}$ performs worse. All methods are
averaged over 10 runs, and error bars represent one standard error.  In (c) we
show the average number of \texttt{pp.gen} calls per evaluation of $\hat{a}$,
and see that the multi-fidelity method maintains similar performance as the
high fidelity method while reducing the number of calls.
\label{fig:mf}
}
\end{center}
\end{figure*}
}

